PLANRL: A Motion Planning and Imitation Learning Framework to Bootstrap Reinforcement Learning

Reinforcement Learning (RL) has shown remarkable progress in simulation environments, yet its application to real-world robotic tasks remains limited due to challenges in exploration and generalization. To address these issues, we introduce PLANRL, a framework that chooses when the robot should use classical motion planning and when it should learn a policy. To further improve the efficiency in exploration, we use imitation data to bootstrap the exploration. PLANRL dynamically switches between two modes of operation: reaching a waypoint using classical techniques when away from the objects and reinforcement learning for fine-grained manipulation control when about to interact with objects. PLANRL architecture is composed of ModeNet for mode classification, NavNet for waypoint prediction, and InteractNet for precise manipulation. By combining the strengths of RL and Imitation Learning (IL), PLANRL improves sample efficiency and mitigates distribution shift, ensuring robust task execution. We evaluate our approach across multiple challenging simulation environments and real-world tasks, demonstrating superior performance in terms of adaptability, efficiency, and generalization compared to existing methods. In simulations, PLANRL surpasses baseline methods by 10-15\% in training success rates at 30k samples and by 30-40\% during evaluation phases. In real-world scenarios, it demonstrates a 30-40\% higher success rate on simpler tasks compared to baselines and uniquely succeeds in complex, two-stage manipulation tasks. Datasets and supplementary materials can be found on our {https://raaslab.org/projects/NAVINACT/}.

==> root/author.tex <==
% %%%%%%%%%%%%%%%%%%%% author.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % sample root file for your "contribution" to a proceedings volume
% %
% % Use this file as a template for your own input.
% %
% %%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \documentclass[a4paper]{article}

% \documentclass{../styles/svproc}
% \usepackage[a4paper]{geometry}
% \usepackage{geometry}
% \geometry{
%     left=1.847in,
%     right=1.569in,
%     top=1.264in,
%     bottom=2.444in,
%     twoside=false
% }

% \usepackage{wrapfig}
% \usepackage[font=small,labelfont=bf]{caption} 
% % RECOMMENDED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{graphicx}
% \usepackage{amssymb}
% \usepackage{amsmath}
% % to typeset URLs, URIs, and DOIs
% \usepackage{url}
% \def\UrlFont{\rmfamily}
% \usepackage[colorlinks]{hyperref}
% \usepackage{subcaption}

% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage[dvipsnames]{xcolor}
% \usepackage{cite}
% \usepackage{placeins}

% \begin{document}
% \mainmatter              % start of a contribution
% %
% % \title{MERGE :Manipulation and Exploration with Reinforced Guidance and Execution }
% % \title{NAVINACT: Merging Navigation and Interaction Networks for Efficient Robotic Learning}
% \title{NAVINACT: Combining Navigation and Imitation Learning for Bootstrapping Reinforcement Learning}
% %
% \titlerunning{NAVINACT}  % abbreviated title (for running head)
% %                                     also used for the TOC unless
% %                                   \toctitle is used
% \newcommand{\NAVINACT}{\textsc{NAVINACT}}
% \newcommand{\todo}[1]{\textcolor{red}{TODO:#1}}
% \bibliographystyle{spbasic} % or another style suitable for Springer
% \bibliography{bibliography} % This tells LaTeX the .bib file location
% \author{Amisha Bhaskar \and Zahiruddin Mahammad \and
% Sachin R Jadhav  \and \\ 
% Pratap Tokekar}
% %
% \authorrunning{Bhaskar et al.,} % abbreviated author list (for running head)
% %
% %%%% list of authors for the TOC (use if author list has to be modified)
% \tocauthor{Amisha Bhaskar, Zahir Mahammed, Sachin Jadhav, and Pratap Tokekar}
% %
% \institute{University of Maryland, College Park MD 20742, USA\\
% \email{\{amishab,zahirmd,sjd3333,tokekar\}@umd.edu}}
% % ,\\ WWW home page:
% % \texttt{http://users/\homedir iekeland/web/welcome.html}
% % \and
% % Universit\'{e} de Paris-Sud,
% % Laboratoire d'Analyse Num\'{e}rique, B\^{a}timent 425,\\
% % F-91405 Orsay Cedex, France}

% \maketitle              % typeset the title of the contribution
% \thispagestyle{empty}
% \pagestyle{empty}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{sections/0.abstract}
% \input{sections/1.introduction}
% \input{sections/2.related_work}
% % \input{sections/3.preliminaries}
% \input{sections/4.proposed_approach}
% \input{sections/5.experiments}
% \input{sections/6.conclusion}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






% %
% % ---- Bibliography ----
% \begin{thebibliography}{6}
% %
% % \bibitem{ros}
% % S. Ross, G. Gordon, and D. Bagnell.: A reduction of imitation learning and structured prediction to no-regret online learning. In Proceedings of the fourteenth international conference
% % on artificial intelligence and statistics, pages 627–635. JMLR Workshop and Conference Proceedings, 2011.
% % \bibitem {smit:wat}
% % Smith, T.F., Waterman, M.S.: Identification of common molecular subsequences.
% % J. Mol. Biol. 147, 195?197 (1981). \url{doi:10.1016/0022-2836(81)90087-5}
% % \bibitem{k_gandhi}
% % Gandhi, Kanishk, Siddharth Karamcheti, Madeline Liao, and Dorsa Sadigh.: "Eliciting compatible demonstrations for multi-human imitation learning." In Conference on Robot Learning, pp. 1981-1991. PMLR, 2023.

% % \bibitem{y_cui}
% % Cui, Yuchen, David Isele, Scott Niekum, and Kikuo Fujimura.: "Uncertainty-aware data aggregation for deep imitation learning." In 2019 International Conference on Robotics and Automation (ICRA), pp. 761-767. IEEE, 2019.

% % \bibitem{r_hoque}
% % Hoque, Ryan, Ashwin Balakrishna, Ellen Novoseller, Albert Wilcox, Daniel S. Brown, and Ken Goldberg.: "Thriftydagger: Budget-aware novelty and risk gating for interactive imitation learning." arXiv preprint arXiv:2109.08273 (2021).

% % \bibitem{m_kelly}
% % Kelly, Michael, Chelsea Sidrane, Katherine Driggs-Campbell, and Mykel J. Kochenderfer.: "Hg-dagger: Interactive imitation learning with human experts." In 2019 International Conference on Robotics and Automation (ICRA), pp. 8077-8083. IEEE, 2019.

% % \bibitem{m_mandlekar}
% % Mandlekar, Ajay, Danfei Xu, Roberto Martín-Martín, Yuke Zhu, Li Fei-Fei, and Silvio Savarese.: "Human-in-the-loop imitation learning using remote teleoperation." arXiv preprint arXiv:2012.06733 (2020).

% % \bibitem{m_l_schrum}
% % Schrum, Mariah L., Erin Hedlund-Botti, Nina Moorman, and Matthew C. Gombolay.: "Mind meld: Personalized meta-learning for robot-centric imitation learning." In 2022 17th ACM/IEEE International Conference on Human-Robot Interaction (HRI), pp. 157-165. IEEE, 2022.

% % \bibitem{laskey_et_al}
% % Laskey, Michael, Jonathan Lee, Roy Fox, Anca Dragan, and Ken Goldberg.: "Dart: Noise injection for robust imitation learning." In Conference on robot learning, pp. 143-156. PMLR, 2017.

% \bibitem{zhu}
% Zhu, Yifeng, Abhishek Joshi, Peter Stone, and Yuke Zhu.: ``Viola: Imitation learning for vision-based manipulation with object proposal priors." In Conference on Robot Learning, pp. 1199-1210. PMLR, 2023.

% \bibitem{s_karamcheti}
% Karamcheti, Siddharth, Suraj Nair, Annie S. Chen, Thomas Kollar, Chelsea Finn, Dorsa Sadigh, and Percy Liang.: ``Language-driven representation learning for robotics." arXiv preprint arXiv:2302.12766 (2023).

% \bibitem{s_nair}
% Nair, Suraj, Aravind Rajeswaran, Vikash Kumar, Chelsea Finn, and Abhinav Gupta.: ``R3m: A universal visual representation for robot manipulation." arXiv preprint arXiv:2203.12601 (2022).

% \bibitem{pertsch}
% Pertsch, Karl, Youngwoon Lee, and Joseph Lim.: ``Accelerating reinforcement learning with learned skill priors." In Conference on robot learning, pp. 188-204. PMLR, 2021.


% \bibitem{lava}
% Bhaskar, Amisha, Rui Liu, Vishnu D. Sharma, Guangyao Shi, and Pratap Tokekar. : "Lava: Long-horizon visual action based food acquisition." arXiv preprint arXiv:2403.12876 (2024).

% \bibitem{pegMARL}
% Yu, Peihong, Manav Mishra, Alec Koppel, Carl Busart, Priya Narayan, Dinesh Manocha, Amrit Bedi, and Pratap Tokekar. : "Beyond Joint Demonstrations: Personalized Expert Guidance for Efficient Multi-Agent Reinforcement Learning." arXiv preprint arXiv:2403.08936 (2024).
% % \bibitem{avil}
% % Liu, Rui, Amisha Bhaskar, and Pratap Tokekar. "Adaptive visual imitation learning for robotic assisted feeding across varied bowl configurations and food types." arXiv preprint arXiv:2403.12891 (2024).



% \bibitem{lynch}
% Lynch, Corey, Mohi Khansari, Ted Xiao, Vikash Kumar, Jonathan Tompson, Sergey Levine, and Pierre Sermanet.: ``Learning latent plans from play." In Conference on robot learning, pp. 1113-1132. PMLR, 2020.



% \bibitem{belkhale}
% Belkhale, Suneel, and Dorsa Sadigh.: ``Plato: Predicting latent affordances through object-centric play." In Conference on Robot Learning, pp. 1424-1434. PMLR, 2023.


% \bibitem{shridhar}
% Shridhar, Mohit, Lucas Manuelli, and Dieter Fox.: ``Perceiver-actor: A multi-task transformer for robotic manipulation." In Conference on Robot Learning, pp. 785-799. PMLR, 2023.
% \bibitem{rlpd}
% Ball, Philip J., Laura Smith, Ilya Kostrikov, and Sergey Levine.: ``Efficient online reinforcement learning with offline data." In International Conference on Machine Learning, pp. 1577-1594. PMLR, 2023.

% \bibitem{akgun}
% Akgun, Baris, Maya Cakmak, Karl Jiang, and Andrea L. Thomaz.: ``Keyframe-based learning from demonstration: Method and evaluation." International Journal of Social Robotics 4 (2012): 343-355.


% \bibitem{chi}
% Chi, Cheng, Siyuan Feng, Yilun Du, Zhenjia Xu, Eric Cousineau, Benjamin Burchfiel, and Shuran Song.: ``Diffusion policy: Visuomotor policy learning via action diffusion." arXiv preprint arXiv:2303.04137 (2023).


% \bibitem{lee_et_al}
% Lee, Michelle A., Carlos Florensa, Jonathan Tremblay, Nathan Ratliff, Animesh Garg, Fabio Ramos, and Dieter Fox.: ``Guided uncertainty-aware policy optimization: Combining learning and model-based strategies for sample-efficient policy learning." In 2020 IEEE international conference on robotics and automation (ICRA), pp. 7505-7512. IEEE, 2020.

% \bibitem{yamada}
% Yamada, Jun, Youngwoon Lee, Gautam Salhotra, Karl Pertsch, Max Pflueger, Gaurav Sukhatme, Joseph Lim, and Peter Englert.: ``Motion planner augmented reinforcement learning for robot manipulation in obstructed environments." In Conference on Robot Learning, pp. 589-603. PMLR, 2021.

% \bibitem{cheng}
% Cheng, Shuo, and Danfei Xu.: ``League: Guided skill learning and abstraction for long-horizon manipulation." IEEE Robotics and Automation Letters (2023).

% \bibitem{xia_et_at}
% Xia, Fei, Chengshu Li, Roberto Martín-Martín, Or Litany, Alexander Toshev, and Silvio Savarese.: ``Relmogen: Leveraging motion generation in reinforcement learning for mobile manipulation." arXiv preprint arXiv:2008.07792 (2020).

% \bibitem{james_davison}
% James, Stephen, and Andrew J. Davison.: ``Q-attention: Enabling efficient learning for vision-based robotic manipulation." IEEE Robotics and Automation Letters 7, no. 2 (2022): 1612-1619.

% \bibitem{james_et_al}
% James, Stephen, Kentaro Wada, Tristan Laidlow, and Andrew J. Davison.: ``Coarse-to-fine q-attention: Efficient learning for visual robotic manipulation via discretisation." In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 13739-13748. 2022.

% \bibitem{liu_et_al}
% Liu, I-Chun Arthur, Shagun Uppal, Gaurav S. Sukhatme, Joseph J. Lim, Peter Englert, and Youngwoon Lee.: ``Distilling motion planner augmented policies into visual control policies for robot manipulation." In Conference on Robot Learning, pp. 641-650. PMLR, 2022.


% \bibitem{red_q}
% Chen, Xinyue, Che Wang, Zijian Zhou, and Keith Ross.: ``Randomized ensembled double q-learning: Learning fast without a model." arXiv preprint arXiv:2101.05982 (2021).


% \bibitem{silver}
% Silver, David, Julian Schrittwieser, Karen Simonyan, Ioannis Antonoglou, Aja Huang, Arthur Guez, Thomas Hubert et al.,: ``Mastering the game of go without human knowledge." nature 550, no. 7676 (2017): 354-359.

% \bibitem{oriol}
% Vinyals, Oriol, Igor Babuschkin, Wojciech M. Czarnecki, Michaël Mathieu, Andrew Dudzik, Junyoung Chung, David H. Choi et al.,: ``Grandmaster level in StarCraft II using multi-agent reinforcement learning." nature 575, no. 7782 (2019): 350-354.

% \bibitem{fair}
% Meta Fundamental AI Research Diplomacy Team (FAIR)†, Anton Bakhtin, Noam Brown, Emily Dinan, Gabriele Farina, Colin Flaherty, Daniel Fried et al.,: ``Human-level play in the game of Diplomacy by combining language models with strategic reasoning." Science 378, no. 6624 (2022): 1067-1074.

% \bibitem{dropout_q}
% Hiraoka, Takuya, Takahisa Imagawa, Taisei Hashimoto, Takashi Onishi, and Yoshimasa Tsuruoka.: ``Dropout q-functions for doubly efficient reinforcement learning." arXiv preprint arXiv:2110.02034 (2021).

% \bibitem{denis}
% Yarats, Denis, Rob Fergus, Alessandro Lazaric, and Lerrel Pinto.: ``Mastering visual continuous control: Improved data-augmented reinforcement learning." arXiv preprint arXiv:2107.09645 (2021).

% \bibitem{Kumar}
% Kumar, Aviral, Anikait Singh, Frederik Ebert, Mitsuhiko Nakamoto, Yanlai Yang, Chelsea Finn, and Sergey Levine. : ``Pre-training for robots: Offline rl enables learning new tasks from a handful of trials." arXiv preprint arXiv:2210.05178 (2022).

% \bibitem{Brohan} 
% Brohan, Anthony, Noah Brown, Justice Carbajal, Yevgen Chebotar, Joseph Dabis, Chelsea Finn, Keerthana Gopalakrishnan et al., :``Rt-1: Robotics transformer for real-world control at scale." arXiv preprint arXiv:2212.06817 (2022).


% \bibitem{ibrl} 
% Hu, Hengyuan, Suvir Mirchandani, and Dorsa Sadigh.: ``Imitation Bootstrapped Reinforcement Learning." arXiv preprint arXiv:2311.02198 (2023).

% \bibitem{hydra} 
% Belkhale, Suneel, Yuchen Cui, and Dorsa Sadigh. ``Hydra: Hybrid robot actions for imitation learning." In Conference on Robot Learning, pp. 2113-2133. PMLR, 2023.

% \bibitem{planseq} 
% Dalal, Murtaza, Tarun Chiruvolu, Devendra Chaplot, and Ruslan Salakhutdinov. ``Plan-seq-learn: Language model guided rl for solving long horizon robotics tasks." arXiv preprint arXiv:2405.01534 (2024).

% \bibitem{rlpd}
% Ball, Philip J., Laura Smith, Ilya Kostrikov, and Sergey Levine. ``Efficient online reinforcement learning with offline data." In International Conference on Machine Learning, pp. 1577-1594. PMLR, 2023.


% \bibitem{hester}
% Hester, Todd, Matej Vecerik, Olivier Pietquin, Marc Lanctot, Tom Schaul, Bilal Piot, Dan Horgan et al., ``Deep q-learning from demonstrations." In Proceedings of the AAAI conference on artificial intelligence, vol. 32, no. 1. 2018.

% \bibitem{nair_ashvin}
% Nair, Ashvin, Bob McGrew, Marcin Andrychowicz, Wojciech Zaremba, and Pieter Abbeel. ``Overcoming exploration in reinforcement learning with demonstrations." In 2018 IEEE international conference on robotics and automation (ICRA), pp. 6292-6299. IEEE, 2018.

% \bibitem{complex_dexterous}
% Rajeswaran, Aravind, Vikash Kumar, Abhishek Gupta, Giulia Vezzani, John Schulman, Emanuel Todorov, and Sergey Levine. ``Learning complex dexterous manipulation with deep reinforcement learning and demonstrations." arXiv preprint arXiv:1709.10087 (2017).


% \bibitem{task_level}
% Seo, Younggyo, Danijar Hafner, Hao Liu, Fangchen Liu, Stephen James, Kimin Lee, and Pieter Abbeel. ``Masked world models for visual control." In Conference on Robot Learning, pp. 1332-1344. PMLR, 2023.


% \bibitem{gello}
% Wu, Philipp, Yide Shentu, Zhongke Yi, Xingyu Lin, and Pieter Abbeel. ``Gello: A general, low-cost, and intuitive teleoperation framework for robot manipulators." arXiv preprint arXiv:2309.13037 (2023).


% \bibitem{metaworld}
% Yu, Tianhe, Deirdre Quillen, Zhanpeng He, Ryan Julian, Karol Hausman, Chelsea Finn, and Sergey Levine. ``Meta-world: A benchmark and evaluation for multi-task and meta reinforcement learning." In Conference on robot learning, pp. 1094-1100. PMLR, 2020.

% \bibitem{td3}
% Dankwa, Stephen, and Wenfeng Zheng. ``Twin-delayed ddpg: A deep reinforcement learning technique to model a continuous movement of an intelligent robot agent." In Proceedings of the 3rd international conference on vision, image and signal processing, pp. 1-5. 2019.

% \bibitem{AT}
% Strub, Marlin P., and Jonathan D. Gammell.: ``Adaptively Informed Trees (AIT*): Fast asymptotically optimal path planning through adaptive heuristics." In 2020 IEEE International Conference on Robotics and Automation (ICRA), pp. 3191-3198. IEEE, 2020.
% \end{thebibliography}



% \end{document}


==> root/sections/3.preliminaries.tex <==
\section{Preliminaries}
 \label{section:preliminaries}


We consider a standard Markov decision process (MDP) consisting of state space $s \in \mathcal{S}$, continuous action space $\mathcal{A} = [-1, 1]^d$, deterministic state transition function $T : \mathcal{S} \times \mathcal{A} \to \mathcal{S}$, sparse reward function $R : \mathcal{S} \times \mathcal{A} \to \{0, 1\}$ that returns 1 when the task is completed and 0 otherwise, and discount factor $\gamma$.



\subsection{Reinforcement Learning}
{\NAVINACT{}} builds upon off-policy RL methods that efficiently leverage demonstration data generated by humans. In deep RL, policies (actors) $\pi_\theta$ and value functions (critics) $Q_\phi$ are represented by neural networks parameterized by $\theta$ and $\phi$. The critic is trained to minimize the temporal difference (TD) error:
\[
L(\phi) = [r_t + \gamma Q_{\phi'}(s_{t+1}, \pi_{\theta'}(s_{t+1})) - Q_\phi(s_t, a_t)]^2,
\]
while the policy is optimized to produce actions that yield high Q-values:
\[
L(\theta) = -Q_\phi(s, \pi_\theta(s)).
\]
Here, $\pi_{\theta'}$ and $Q_{\phi'}$ are target networks, with parameters $\theta'$ and $\phi'$ being exponential moving averages of $\theta$ and $\phi$, respectively.

\subsection{Imitation Learning}
Imitation learning (IL) assumes access to a dataset $\mathcal{D}$ consisting of expert demonstrations. Each trajectory $\xi \in \mathcal{D}$ is a sequence of state-action pairs $\{(s_0, a_0), \ldots, (s_T, a_T)\}$. The most common IL approach is behavior cloning (BC), which trains a policy $\mu_\psi$ to minimize the negative log-likelihood of the demonstrated actions:
\[
L(\psi) = -\mathbb{E}_{(s,a)\sim\mathcal{D}}[\log \mu_\psi(a|s)].
\]
Assuming $\mu_\psi$ follows an isotropic Gaussian distribution, the BC training objective can be expressed as:
\[
L(\psi) = \mathbb{E}_{(s,a)\sim\mathcal{D}} \|\mu_\psi(s) - a\|_2^2.
\]

\subsection{Distribution Shift in IL}
A key challenge in IL is distribution shift between training and deployment, where small errors in action selection can lead to significant deviations in state trajectories. To mitigate this, our approach incorporates a hybrid action space that combines high-level waypoint navigation with precise low-level control, ensuring consistency and reducing the impact of distribution shift during real-world execution.





